Toward Interactive Regional Understanding in Vision-Large Language Models

Recent Vision-Language Pre-training (VLP) models have demonstrated significant advancements. Nevertheless, these models heavily rely on image-text pairs that capture only coarse and global information of an image, leading to a limitation in their regional understanding ability. In this work, we introduce \textbf{RegionVLM}, equipped with explicit regional modeling capabilities, allowing them to understand user-indicated image regions. To achieve this, we design a simple yet innovative architecture, requiring no modifications to the model architecture or objective function. Additionally, we leverage a dataset that contains a novel source of information, namely Localized Narratives, which has been overlooked in previous VLP research. Our experiments demonstrate that our single generalist model not only achieves an interactive dialogue system but also exhibits superior performance on various zero-shot region understanding tasks, without compromising its ability for global image understanding.

==> __unused.tex <==
These instructions are for authors submitting papers to *ACL conferences using \LaTeX. They are not self-contained. All authors must follow the general instructions for *ACL proceedings,\footnote{\url{http://acl-org.github.io/ACLPUB/formatting.html}} and this document contains additional instructions for the \LaTeX{} style files.

The templates include the \LaTeX{} source of this document (\texttt{acl.tex}),
the \LaTeX{} style file used to format it (\texttt{acl.sty}),
an ACL bibliography style (\texttt{acl\_natbib.bst}),
an example bibliography (\texttt{custom.bib}),
and the bibliography for the ACL Anthology (\texttt{anthology.bib}).

\section{Engines}

To produce a PDF file, pdf\LaTeX{} is strongly recommended (over original \LaTeX{} plus dvips+ps2pdf or dvipdf). Xe\LaTeX{} also produces PDF files, and is especially suitable for text in non-Latin scripts.

\section{Preamble}

The first line of the file must be
\begin{quote}
\begin{verbatim}
\documentclass[11pt]{article}
\end{verbatim}
\end{quote}

To load the style file in the review version:
\begin{quote}
\begin{verbatim}
\usepackage[review]{acl}
\end{verbatim}
\end{quote}
For the final version, omit the \verb|review| option:
\begin{quote}
\begin{verbatim}
\usepackage{acl}
\end{verbatim}
\end{quote}

To use Times Roman, put the following in the preamble:
\begin{quote}
\begin{verbatim}
\usepackage{times}
\end{verbatim}
\end{quote}
(Alternatives like txfonts or newtx are also acceptable.)

Please see the \LaTeX{} source of this document for comments on other packages that may be useful.

Set the title and author using \verb|\title| and \verb|\author|. Within the author list, format multiple authors using \verb|\and| and \verb|\And| and \verb|\AND|; please see the \LaTeX{} source for examples.

By default, the box containing the title and author names is set to the minimum of 5 cm. If you need more space, include the following in the preamble:
\begin{quote}
\begin{verbatim}
\setlength\titlebox{<dim>}
\end{verbatim}
\end{quote}
where \verb|<dim>| is replaced with a length. Do not set this length smaller than 5 cm.

\section{Document Body}

\subsection{Footnotes}

Footnotes are inserted with the \verb|\footnote| command.\footnote{This is a footnote.}

\subsection{Tables and figures}

See Table~\ref{tab:accents} for an example of a table and its caption.
\textbf{Do not override the default caption sizes.}

\begin{table}
\centering
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\"a}| & {\"a} \\
\verb|{\^e}| & {\^e} \\
\verb|{\`i}| & {\`i} \\ 
\verb|{\.I}| & {\.I} \\ 
\verb|{\o}| & {\o} \\
\verb|{\'u}| & {\'u}  \\ 
\verb|{\aa}| & {\aa}  \\\hline
\end{tabular}
\begin{tabular}{lc}
\hline
\textbf{Command} & \textbf{Output}\\
\hline
\verb|{\c c}| & {\c c} \\ 
\verb|{\u g}| & {\u g} \\ 
\verb|{\l}| & {\l} \\ 
\verb|{\~n}| & {\~n} \\ 
\verb|{\H o}| & {\H o} \\ 
\verb|{\v r}| & {\v r} \\ 
\verb|{\ss}| & {\ss} \\
\hline
\end{tabular}
\caption{Example commands for accented characters, to be used in, \emph{e.g.}, Bib\TeX{} entries.}
\label{tab:accents}
\end{table}

\subsection{Hyperlinks}

Users of older versions of \LaTeX{} may encounter the following error during compilation: 
\begin{quote}
\tt\verb|\pdfendlink| ended up in different nesting level than \verb|\pdfstartlink|.
\end{quote}
This happens when pdf\LaTeX{} is used and a citation splits across a page boundary. The best way to fix this is to upgrade \LaTeX{} to 2018-12-01 or later.

\subsection{Citations}

\begin{table*}
\centering
\begin{tabular}{lll}
\hline
\textbf{Output} & \textbf{natbib command} & \textbf{Old ACL-style command}\\
\hline
\citep{Gusfield:97} & \verb|\citep| & \verb|\cite| \\
\citealp{Gusfield:97} & \verb|\citealp| & no equivalent \\
\citet{Gusfield:97} & \verb|\citet| & \verb|\newcite| \\
\citeyearpar{Gusfield:97} & \verb|\citeyearpar| & \verb|\shortcite| \\
\hline
\end{tabular}
\caption{\label{citation-guide}
Citation commands supported by the style file.
The style is based on the natbib package and supports all natbib citation commands.
It also supports commands defined in previous ACL style files for compatibility.
}
\end{table*}

\citep{alayrac2022flamingo}
Table~\ref{citation-guide} shows the syntax supported by the style files.
We encourage you to use the natbib styles.
You can use the command \verb|\citet| (cite in text) to get ``author (year)'' citations, like this citation to a paper by \citet{Gusfield:97}.
You can use the command \verb|\citep| (cite in parentheses) to get ``(author, year)'' citations \citep{Gusfield:97}.
You can use the command \verb|\citealp| (alternative cite without parentheses) to get ``author, year'' citations, which is useful for using citations within parentheses (e.g. \citealp{Gusfield:97}).

\subsection{References}

\nocite{Ando2005,andrew2007scalable,rasooli-tetrault-2015}

The \LaTeX{} and Bib\TeX{} style files provided roughly follow the American Psychological Association format.
If your own bib file is named \texttt{custom.bib}, then placing the following before any appendices in your \LaTeX{} file will generate the references section for you:
\begin{quote}
\begin{verbatim}
\bibliography{custom}
\end{verbatim}
\end{quote}

You can obtain the complete ACL Anthology as a Bib\TeX{} file from \url{https://aclweb.org/anthology/anthology.bib.gz}.
To include both the Anthology and your own .bib file, use the following instead of the above.
\begin{quote}
\begin{verbatim}
\bibliography{anthology,custom}
\end{verbatim}
\end{quote}

Please see Section~\ref{sec:bibtex} for information on preparing Bib\TeX{} files.

\subsection{Appendices}

Use \verb|\appendix| before any appendix section to switch the section numbering over to letters. See Appendix~\ref{sec:appendix} for an example.

\section{Bib\TeX{} Files}
\label{sec:bibtex}

Unicode cannot be used in Bib\TeX{} entries, and some ways of typing special characters can disrupt Bib\TeX's alphabetization. The recommended way of typing special characters is shown in Table~\ref{tab:accents}.

Please ensure that Bib\TeX{} records contain DOIs or URLs when possible, and for all the ACL materials that you reference.
Use the \verb|doi| field for DOIs and the \verb|url| field for URLs.
If a Bib\TeX{} entry has a URL or DOI field, the paper title in the references section will appear as a hyperlink to the paper, using the hyperref \LaTeX{} package.

\section*{Acknowledgements}

This document has been adapted
by Steven Bethard, Ryan Cotterell and Rui Yan
from the instructions for earlier ACL and NAACL proceedings, including those for 
ACL 2019 by Douwe Kiela and Ivan Vuli\'{c},
NAACL 2019 by Stephanie Lukin and Alla Roskovskaya, 
ACL 2018 by Shay Cohen, Kevin Gimpel, and Wei Lu, 
NAACL 2018 by Margaret Mitchell and Stephanie Lukin,
Bib\TeX{} suggestions for (NA)ACL 2017/2018 from Jason Eisner,
ACL 2017 by Dan Gildea and Min-Yen Kan, 
NAACL 2017 by Margaret Mitchell, 
ACL 2012 by Maggie Li and Michael White, 
ACL 2010 by Jing-Shin Chang and Philipp Koehn, 
ACL 2008 by Johanna D. Moore, Simone Teufel, James Allan, and Sadaoki Furui, 
ACL 2005 by Hwee Tou Ng and Kemal Oflazer, 
ACL 2002 by Eugene Charniak and Dekang Lin, 
and earlier ACL and EACL formats written by several people, including
John Chen, Henry S. Thompson and Donald Walker.
Additional elements were taken from the formatting instructions of the \emph{International Joint Conference on Artificial Intelligence} and the \emph{Conference on Computer Vision and Pattern Recognition}.


==> introduction_old.tex <==

With the advent of large-scale image-text pair datasets \cite{schuhmann2021laion,schuhmann2022laion_5b,gadre2023datacomp} and the advanced Transformer architectures~\citep{vaswani2017attention}, research on Vision-Language Pre-training (VLP) has recently made significant progress. Most VLP models are trained on vast quantities of image-text pairs, which can be automatically obtained from the web. These pairs are highly diverse and expressive, enabling the learning of a general and meaningful vision-language representation. 
Therefore, foundation models with zero-shot capability have emerged, where a single generalist model excels in various vision-language downstream tasks, such as visual question answering and image classification, without the need for training data for finetuning each task.
In particular, VLP models leveraging the frozen Large Language Models (LLMs) have demonstrated their zero-shot and few-shot superiority, fully harnessing the generality power of LLMs~\cite{li2023blip2, alayrac2022flamingo, koh2023grounding}.
% by fully utilizing the generality power of LLMs~\cite{li2023blip2, alayrac2022flamingo}.



% from a single generalist (foundation) model.
% 따라서, 하나의 generalist (foundation) 모델로 여러 다양한 Downstream-task에 zero-shot 개쩌는 모델들 나왔음 (such as VQA and image classification).
% These models, serving as a single generalist (foundation) model, excel in various downstream tasks with zero-shot capability, such as Visual Question Answering (VQA) and image classification.

% web에서 자동적으로 얻을 수 있는 방대한 양의 image-text pair dataset 과 advanced Transfoermer architecture 의 발전으로 Vision-language pre-training (VLP) research 는 최근 매우 크게 발전해왔다. 
% web 에서 얻어지는 image-text pair는 매우 다양하고 expressive 하여 매우 general 하고 meaningful 한 shared representation 을 학습한다.
% 이러한 모델들은 하나의 generalist (foundation) 모델로 여러 다양한 Downstream-task에 zero-shot 개쩜 (such as VQA and image classification). 

% 현재까지 VLP 방법론들은 global image - global caption matching 에 집중 해와서 global image 와 caption 사이의 shared,  representation 학습했음.
% 그로부터 다양한 downstream task가 가능 했지만, local 한 정보를 필요로 하는 task 들은 수행 불가. 
% 특히  으로 가속화?


% [region understanding 의 중요성]
However, existing image-text pairs tend to focus on the global and salient information of the image and do not provide an explicit indication of which part of the image the text is describing.
Therefore, the existing VLP models trained on such pairs lack the ability to comprehend fine-grained semantics for specified regions (\eg, user input location) in the image.
\textcolor{blue}{The region understanding capability of the VLP model is paramount for the following reasons:
First, this makes VLP model more versatile by enabling the execution of additional vision-language tasks that necessitate the explicit indication of regions, such as referring image segmentation and visual commonsense reasoning.
% Second, 
% explicit region indication이 필요한 다양한 task 더 풀 수 있음 
Second, it tackles ambiguities inherent in visual-language tasks that the current VLP models are actively handling.
For example, when trying to inquire about a specific object within an image, the current system may specify it solely using texts, which can introduce ambiguity.
% For example, 이미지 내의 특정 영역을 specify 하고 싶을 때, text 로 설명해야 하는데 이게 좀 애매할 수 있음
% Third, we can develop an interactive model 
Third, this enhances interactivity between the model and the user, aligning with the desirable research direction exemplified in GPT-4V~\cite{gpt4v, yang2023dawn}.}
% user와의 interactive 한 system 더 versatile, evidenced by GPT-4V visual referring prompting function~\cite{yang2023dawn}.

% and exhibit limited scalability for tasks that require explicit region understanding abilities, such as referring image segmentation and visual commonsense reasoning.
% \textcolor{red}{region understanding ability의 중요성이 더 강조되면 좋을 것 같은데..}

% local region 에 대한 Understanding 이 부족하다.


% \input{Figures/Figure1}
% \input{Figures/LN_examples}



% they have no indication where the text describes on the image
% 게다가 local한 정보를 본다 해도 어디를 indicate 하는지 모른다?
% Especially, selectively modeling information related to the specific (target) region is challenging.
% The region understanding ability of the VLP model is crucial. This is because 1) it enables handling numerous downstream tasks that require modeling of regional information (\textit{e.g.,} referring image segmentation and visual commonsense reasoning), making the VLP model more versatile. 
% % object detection, segmentation, referring, VCR), making the VLP model more versatile. 
% \textcolor{red}{2) Global captions tend to focus on the salient regions of the image, but lack fine-grained details. 
% global image task인 VQA에서도 fine-grained detail 이 중요할때가 있다? Fine-grained information is often helpful. Even for VQA, a lot of fine-grained information is needed.}

% 현존하는 image-text pair 는 image 의 global 정보만을 고려하기 때문에, VLP 모델들은 fine-grained understanding ability가 부족함. 특히 target region 에 관련된 정보를 modeling 하는 것이 unfeasible. 
% VLP model의 region understanding ability 는 crucial. 왜냐하면 1) region 정보를 modeling 해야 하는 수많은 task들까지 가능해져서 더 versatile 해짐 (detection, segmentation, referring, VCR). 2) global caption 은 주로 이미지의 salient 한 부분에 집중하고 fine-grained 한 정보 모델링 안함. 하지만 이런 fine-grained 정보가 도움이 될 때가 많음. VQA 만 해도 fine-grained 정보 많이 필요함



% \input{Figures/LN_examples}


% [간단한 related work과 단점] 
Several efforts have been made to endow VLP models with region understanding ability.
% Starting from a generalist model that lacks region understanding ability, some methods~\citep{zhou2023zegclip, gu2021open, yun2023ifseg, li2023tagclip} focus on developing specialized models for specific region understanding tasks, such as segmentation and detection, by using fully supervised labels for each task.
Built upon a generalist model lacking region understanding ability (\eg, CLIP~\cite{radford2021learning}), some methods~\citep{zhou2023zegclip, gu2021open, yun2023ifseg, li2023tagclip} have developed specialized models for region understanding tasks, such as segmentation and detection, by utilizing fully supervised labels for each task.
Very recently, there have been studies aiming to create a generalist model capable of region understanding~\citep{zhang2023gpt4roi, wang2023visionllm, jin2023grill, zhou2023regionblip}.
To achieve this, a dataset containing image regions with their corresponding captions is essential. However, the datasets employed for VLP training thus far have inherent limitations.
% there are limitations in the datasets that have been used for VLP training until now.
% However, they have used the data that has limitations in terms of generality. 
For example, the visual grounding dataset~\citep{yu2016modeling} contains region-text pairs for a limited set of object classes, and the Visual Genome~\citep{krishna2017visual} tends to feature short captions depicting a limited relationship between objects.
% contain short captions depicting the limited relationship between objects.
To achieve generality and scalability in VLP models, a dataset containing diverse regions, indicating various open-world objects, along with expressive captions, is required. 

% dense captions contain sentences with limited expressiveness.
% To achieve versatility and scalability in VLP models, it is imperative to include diverse regions indicating various open-world objects, along with expressive captions.
% is limited to specific classes of target objects, 
% diverse regions indicating various open-world objects along with expressive captions are needed.

% 하지만 그들이 사용한 데이터는 generlity의 한계가 있음. ex: RefCOCO 는 coco object 에 한정, vg는 문장의 표현력 한계, VCR 영역이 주로 사람
% generality 와 unseen task 에 대한 zero-shot ability를 위해선 다양한 Open-world의 region 과 caption이 필요함. 


% 실제로, 기존의 VLP 모델의 region understanding ability의 한계에서 motivation 을 얻어, VLP 모델이 region 정보를 inject 시키려는 시도는 있었음.
% VLP 모델이 region understanding ability 를 부여하려는 노력이 있었음.
% 대부분 fully supervised labels 을 이용해 specialized 모델을 만드는데 집중 for specific tasks such as segmentation and detection.
% Very recently, region understanding 이 가능한 generalist 모델을 만드려는 연구들이 나왔다.

% ~\citep{wang2023visionllm, lai2023lisa, }
% 최근에, 우리의 concurrent work 들. generalist 모델을 만드려는 노력. 하지만 그들이 사용한 데이터는 generlity의 한계가 있음. ex: RefCOCO 는 coco object 에 한정, vg는 문장의 표현력 한계, VCR 영역이 주로 사람
% generality 와 unseen task 에 대한 zero-shot ability를 위해선 다양한 Open-world의 region 과 caption이 필요함. 
% 하지만 그들이 사용한 데이터는 generlity의 한계가 있다. 예를 들면, visual grounding dataset 은 제한적인 종류의 target object 를 가지고 있고, visual genome dense caption 은 표현력의 한계가 있는 문장을 포함한다.


% [우리가 쓸 dataset] 
In this paper, we employ a dataset containing a novel source of information that has been overlooked in previous research. 
% Existing works on VLP use either datasets that are expressive but limited to the global image understanding (\textit{i.e.,} image-text pairs) or datasets that allow for regional understanding but with restricted generality and expressiveness.
We propose to utilize the Localized Narratives dataset~\cite{pont2020connecting, voigtlaender2023connecting} to develop a generalist VLP model that can perform both global and local tasks in a zero-shot manner. 
It provides an image along with the trajectory of mouse pointers generated while an annotator describes the corresponding region.
This dataset is a large-scale dataset that includes expressive free-form captions depicting multiple open-world objects in a single image (Figure~\ref{LN_examples}), and thus it can provide general and meaningful regional information to the VLP model.

% It is large-scale, contains expressive free-form captions depicting multiple objects in a single image, which are open-world.
% The Localized Narratives dataset  because it .



% 기존 work은 expressive 하지만 global understanding만 가능한 데이터셋 사용 (cc3m, laion), 혹은 regional understanding 이 가능하지만 표현력이 제한된 학습 데이터 사용. 이와 달리 We realize the zero-shot generality by using a new source of information for VLP. Localized narrative의 이점: 1) regional understanding with expressive한 표현력 이 가능해짐. 2) localized narrative의 input 형태가 scribble 이므로, 기존의 region input인 box, mask 등에 비해 직관적이면서 빠르고 쉽게 줄 수 있음.

% [proposed model 설명]

% We present a straightforward yet intuitive technique to convey region information to the model. 
% We treat a set of points, supplied by the Localized Narratives dataset, as text and convert it into textual tokens.
% The tokens are then fed into the model.
% By training the model to generate captions for given points, it learns to automatically attend to the corresponding regions for those given points.

We introduce a simple yet intuitive technique to convey regional information obtained from the Localized Narratives dataset to the model. 
We regard a set of trajectory points, provided by the Localized Narratives dataset, as a sequence of strings and convert them into textual tokens. 여기 LLM 얘기 없어도 되나? 제목에 LLM이 들어가면 해야할거같은데
These tokens are subsequently fed into the model together with the entire image.
We then train the model to generate captions for the region corresponding to the given point in the provided image.
As a result, the model learns to automatically direct its focus towards the corresponding regions associated with those points, resulting in an ability to understand regional information.
Our approach does not require architectural modifications to the existing model and seamlessly aligns with the original scheme, which takes both the entire image and text as input. 
Therefore, our model can additionally perform new tasks that require utilizing local information of an image, while retaining its generality for tasks related to the global image.



The main contributions of this paper are summarized as follows.
First, we design a simple yet novel architecture for region understanding without modifying the model architecture.
Second, we propose to utilize a new source of information that has not been explored in Vision-Language pretraining.
Third, we demonstrate that our single generalist model produces superior performance on various zero-shot region understanding tasks without compromising its ability for global image understanding.
% losing the ability of global image understanding ability.
% preserving the superiority while 
% can perform in a zero-shot manner. 
% global task 성능 유지하면서 zero-shot local task 잘함. region understanding required tasks


